Probabilistic Abstractions with Arbitrary Domains

Recent work by Hermanns et al. and Kattenbelt et al. has extended counterexample-guided abstraction refinement (CEGAR) to probabilistic programs. These approaches are limited to predicate abstraction. We present a novel technique, based on the abstract reachability tree recently introduced by Gulavani et al., that can use arbitrary abstract domains and widening operators (in the sense of abstract interpretation). We show how suitable widening operators can deduce loop invariants diffcult to find for predicate abstraction, and propose refinement techniques.

==> intro.tex <==
%
\section{Introduction}
Abstraction techniques are crucial for the automatic verification of systems
with a finite but very large or infinite state space. The
abstract interpretation framework provides the mathematical basis of
abstraction \cite{cousot}. 
Recent work has extended abstraction techniques to probabilistic systems \cite{kattenbelt,wachter}. 
The systems (e.g. probabilistic programs) are given semantics in terms of Markov
Decision Processes (MDPs), which can model nondeterminism and (using interleaving semantics)
concurrency. The key idea is to abstract the MDP into a stochastic 2-player game. 
The two players of the abstraction distinguish between nondeterminism inherent to the system 
(modelled by the choices of player 1)
and nondeterminism introduced by the abstraction (modelled by player 2). 
%When the system is
%sequential and deterministic, player one is not needed; the system 
%is then modelled by a Markov chain, and its abstraction by an MDP.


The construction ensures that the probability of reaching a goal state in the MDP using an
optimal strategy can be bounded from above and from below by computing the
supremum and infimum of the probabilities of reaching the goal in the 2-player game when player
1 plays according to an optimal strategy (and player 2 is free to play in any way).
An analogous result holds for the probability of reaching a goal state in the MDP using a
pessimal strategy.

The abstraction technique of \cite{kattenbelt,wachter} relies on predicate abstraction:
an abstract state is an equivalence class of concrete states, where 
two concrete states are equivalent if they satisfy the same subset of a given
set of predicates. If the upper and lower bounds obtained using a set of predicates
are not close enough, the abstraction can be refined by adding new predicates with the help of
interpolation, analogously to the well-known CEGAR approach for
non-probabilistic systems. 

While predicate abstraction 
has proved very successful, it is known to have a number of shortcomings, like 
potentially expensive equality and inclusion checks for abstract states, and ``predicate explosion''.
In the non-probabilistic case, the work of Gulavani {\it et al.} has 
extended the CEGAR approach to a broader range of abstract domains \cite{gulavani_old}, in which 
widening operations can be combined with interpolation methods, leading to more efficient abstraction algorithms.

In this paper we show that the ideas of Gulavani {\it et al.} can also be applied
in the probabilistic area, resulting in an extension of the approaches of \cite{kattenbelt,wachter} to 
arbitrary abstract domains. Given a probabilistic program, an abstract domain and a widening for this domain, 
we show how to construct a stochastic 2-player game, and how to refine the abstraction using standard 
techniques of abstract interpretation, like delaying widenings \cite{astree}. We also show how this can be done incrementally by ``refining'' special nodes in the game, which can be seen as an
analogon to the refinement techniques in probabilistic CEGAR. Finally, we explain how to derive the
predicate abstraction approach as a special case.

The rest of the paper is organized as follows. In the rest of the introduction we 
informally present the key ideas of our approach by means of some examples. Section \ref{sec:preliminaries}
contains preliminaries. Section \ref{sec:abstraction} formally introduces the abstraction technique, and
proves that the probabilities of the optimal resp. pessimal startegies are an upper resp.
a lower bound of the exact probability of reaching a state. In section \ref{subsec:predabstr} we deal with
the special case of predicate abstraction. Section \ref{sec:experiments} discusses the interest of the 
generalization with the help of some experiments.

\paragraph{Related work.}
Besides the work of~\cite{hermanns} and~\cite{kattenbelt}, 
Monniaux~\cite{monniaux1,monniaux2} has studied how to abstract 
probability distributions over program states (instead of the states themselves).
Wachter et al. discuss in~\cite{probtrans} an abstract-interpretation-based 
framework for analyzing stochastic games, but still rely on predicate abstraction. 



\subsection{An example}
\label{subsec:example}
%     // exit loop if connection closed 
%     //or 100 packages have been sent
We give an informal introduction to our approach by means of an example.
Our main ideas can already be explained in the setting of sequential deterministic programs, 
where the semantics of the program is a Markov chain, and abstractions 
correspond to MDPs. For this reason, we consider 
the C-like program of Fig.~\ref{fig:ex1_code}.
\begin{figure}
\begin{minipage}{5cm}
\begin{verbatim}
   int nrp = 0;

1: while (nrp <= 100)
2:   if (receive_package()) then
3:     nrp = nrp+1
4:   else break 
5: if (nrp < 1) then
6:   fail
7: end.
\end{verbatim}
\end{minipage}
\begin{minipage}{8cm}
%\begin{figure}[htbp]
 \tikzset{
    state/.style={
           rectangle,
           rounded corners,
           draw=black, very thick,
           minimum height=2em,
           inner sep=2pt,
           text centered,
           },
  fail/.style={fill=black,draw=none,text=white},
  nothing/.style={
           rectangle,
           rounded corners,
           minimum height=2em,
           inner sep=0pt,
           text centered,
           }
  }
\scalebox{0.6}{
\begin{tikzpicture}[->,>=stealth',scale=1]
 \node[state, anchor=center] (S1) 
 {L1, \texttt{nrp=0}};
  
 \node[state] (S2) [below =of S1]
 {L2, \texttt{nrp=0}};
 
 \node[state] (S3) [below left=of S2]
  {L3, \texttt{nrp=0}};

 \node[state] (S4) [below =of S3]
  {L1, \texttt{nrp=1}};

 \node[state] (S5) [below =of S4]
  {L2, \texttt{nrp=1}};

 \node[state] (S6) [below left =of S5]
  {L3, \texttt{nrp=1}};

\node[state] (S7) [below right =of S5]
  {L4, \texttt{nrp=1}};

\node[state] (S8) [below =of S7]
  {L5, \texttt{nrp=1}};

\node[fail] (S9) [below =of S8]
  {L7, \texttt{nrp=1}};

\node[state] (S10) [below =of S6]
  {L1, \texttt{nrp=2}};

\node[state] (S11) [below =of S10]
  {L2, \texttt{nrp=2}};

\node[state] (S15) [below right =of S2]
  {L4, \texttt{nrp=0}};

\node[state] (S16) [below =of S15]
  {L5, \texttt{nrp=0}};

\node[fail] (S17) [below =of S16]
  {Fail (L6),\texttt{nrp=0}};

 \node[nothing] (C1)  [below left=of S11]
  { \Large{\dots} };

 \node[nothing] (C2)  [below right=of S11]
  { \Large{\dots} };

 % draw the paths and and print some Text below/above the graph
 \path (S1) edge[right ] node [below right] {$1$} (S2)
       (S2) edge[above]  node{$0.99$} (S3)
       (S2) edge[above]  node{$0.01$} (S15)
       (S15) edge[left]  node{$1$} (S16)
       (S16) edge[left]  node{$1$} (S17)
       (S3) edge[left]  node{$1$} (S4)
       (S4) edge[left]  node{$1$} (S5)
       (S5) edge[above]  node{$0.99$} (S6)
       (S5) edge[above]  node{$0.01$} (S7)
       (S7) edge[left]  node{$1$} (S8)
       (S8) edge[left]  node{$1$} (S9)
       (S6) edge[left]  node{$1$} (S10)
       (S10) edge[left]  node{$1$} (S11)
       (S11) edge[above]  node{$0.99$} (C1)
       (S11) edge[above]  node{$0.01$} (C2);
\end{tikzpicture}
}
%\label{fig:ex1_mc}
%\caption{Prefix of the concrete transition system.}
%\end{figure}
\end{minipage}
\caption{Example program and corresponding transition system.}
\label{fig:ex1_code}
\end{figure}
The goal of the program is to receive $100$ packages. Whenever the program
executes \texttt{receive_package()}, the network connection can be interrupted with probability $0.01$
(\texttt{receive\_package()} returns false) and no further packages can be received.
The probability of receiving no package at all (equal
to the probability of reaching location 6) is obviously $0.01$ (only
the first iteration of the loop is relevant). However, a brute force 
automatic technique will construct and analyze the standard
semantics of the program, a Markov chain with over 400 states, part of which
is shown in Fig.~\ref{fig:ex1_code}. We now informally introduce our abstraction technique, which
also ``sees'' that only the first iteration counts.

A (concrete) state of the program is a pair
$\langle \ell, v \rangle$, where $\ell$ is the current program point and 
$v$ the current value of \texttt{nrp}. We use the abstract interpretation framework \cite{cousot}, 
and choose the \emph{integer interval domain}: an abstract 
state is a pair $\langle \ell, [a, b] \rangle$, where $[a,b]$ is an interval of values of \texttt{npr}.
Starting with $\tup{1, [0,0]}$ we compute successor abstract states in the usual way using depth-first search (DFS):
We compute all direct successors of an abstract state $q$ using the standard 
recipe of abstract interpretation. If one of the successors $d$ has already been generated before, 
we add a transition from $q$ to $d$. Also, if the successors of $q$ are the outcome of a probabilistic 
choice (like at line 2), we label the transitions with probabilities. To keep 
the number of explored abstract states small, we apply a {\em widening operator} $\nabla$:
If we generate an abstract state $\tup{\ell, [a,b]}$ such that 
$\ell$ is the head of a while loop (in our example the only head is $\ell = 1$), 
and $\tup{\ell, [a,b]}$ has an
ancestor $\tup{\ell, [a',b']}$ in the spanning tree generated by the DFS, 
then we overapproximate $\tup{\ell, [a,b]}$ by $\tup{\ell, s}$, with $s =  [a',b']\, \nabla \, [\min(a, a'), \max(b,b')]$. We use the classical widening operator defined
in~\cite{cousot} for this example.
\andreas{Javier: Wideningerklaerung vervollstaendigt. NEIN: widening explizit angeben!!}
To get more precision, 
the use of widenings can be skipped at certain situations. In our example we use $k=1$, 
i.e. we apply widening after the second unrolling of the loop. Moreover, we have to take care of the
fact that abstraction introduces {\em nondeterminism}, since
an abstract state can represent several concrete states. In our case 
this happens at state $\tup{1, [1, \infty)}$: The guard \texttt{nrp <= 100} is satisfied by $[1, 100]$, 
but not satisfied by $[101, \infty)$. In this case we add two successor states, labeled with ''?''.

\begin{figure}[h]
\centering
 \tikzset{
    state/.style={
           rectangle,
           rounded corners,
           draw=black, very thick,
           minimum height=2em,
           inner sep=2pt,
           text centered,
           },
  fail/.style={fill=black,draw=none,text=white},
  nothing/.style={
           rectangle,
           rounded corners,
           minimum height=2em,
           inner sep=0pt,
           text centered,
           }
  }
\scalebox{0.6}{
\begin{tikzpicture}[->,>=stealth',scale=1, font=\large]
 % Position of QUERY 
 % Use previously defined 'state' as layout (see above)
 % use tabular for content to get columns/rows
 % parbox to limit width of the listing
 \node[state, anchor=center] (S1) 
 {L1, $[0,0]$};
  
 \node[state] (S2) [below =of S1]
 {L2, $[0,0]$};
 
 \node[state] (S3) [below left=of S2]
  {L3, $[0,0]$};

 \node[state] (S4) [below =of S3]
  {L1, $[1,1]$};

 \node[state] (S5) [below =of S4]
  {L2, $[1,1]$};

 \node[state] (S6) [below left =of S5]
  {L3, $[1,1]$};

\node[state] (S7) [below right =of S5]
  {L4, $[1,1]$};

\node[state] (S8) [below =of S7]
  {L5, $[1,1]$};

\node[fail] (S9) [below =of S8]
  {L7, $[1,1]$};

\node[state] (S10) [below =of S6]
  {L1, $[1,\infty)$};

\node[state] (S11) [below =of S10]
  {L2, $[1,100]$};

\node[state] (S20) [below left=of S11]
  {L3, $[1, 100]$};

\node[state] (S21) [below right=of S11]
  {L4, $[1, 100]$};

\node[state] (S22) [below =of S21]
  {L5, $[1, 100]$};

\node[fail] (S23) [below =of S22]
  {L7, $[1, 100]$};

\node[state] (S32) [right =of S21]
  {L5, $[101, \infty)$};

\node[fail] (S33) [below =of S32]
  {L7, $[101, \infty)$};

\node[state] (S15) [below right =of S2]
  {L4, $[0,0]$};

\node[state] (S16) [below =of S15]
  {L5, $[0,0]$};

\node[fail] (S17) [below =of S16]
  {Fail (L6),$[0,0]$};

 % draw the paths and and print some Text below/above the graph
 \path (S1) edge[right ] node [below right] {$1$} (S2)
       (S2) edge[above]  node{$0.99$} (S3)
       (S2) edge[above]  node{$0.01$} (S15)
       (S15) edge[left]  node{$1$} (S16)
       (S16) edge[left]  node{$1$} (S17)
       (S3) edge[left]  node{$1$} (S4)
       (S4) edge[left]  node{$1$} (S5)
       (S5) edge[above]  node{$0.99$} (S6)
       (S5) edge[above]  node{$0.01$} (S7)
       (S7) edge[left]  node{$1$} (S8)
       (S8) edge[left]  node{$1$} (S9)
       (S6) edge[left]  node{$1$} (S10)
       (S10) edge[left]  node{$?$} (S11)
       (S11) edge[above]  node{$0.99$} (S20)
       (S11) edge[above]  node{$0.01$} (S21)
       (S20) edge[above]  node{$1$} (S10)
       (S21) edge[left]  node{$1$} (S22)
       (S22) edge[left]  node{$1$} (S23)
       (S10) edge[above]  node{$?$} (S32)
       (S32) edge[left]  node{$1$} (S33);
\end{tikzpicture}
}
\caption{Abstract transition system of the program in Fig.~\ref{fig:ex1_code}.}
\label{fig:ex1_abstr}
\end{figure}
% \begin{minipage}[b]{0.2\linewidth} 
%  
%  \tikzset{
%     state/.style={
%            rectangle,
%            rounded corners,
%            draw=black, very thick,
%            minimum height=2em,
%            inner sep=2pt,
%            text centered,
%            },
%   fail/.style={fill=black,draw=none,text=white},
%   nothing/.style={
%            rectangle,
%            rounded corners,
%            minimum height=2em,
%            inner sep=0pt,
%            text centered,
%            }
%   }
% \scalebox{0.5}{
% \centering
% \begin{tikzpicture}[->,>=stealth',scale=1]
% 
%  % Position of QUERY 
%  % Use previously defined 'state' as layout (see above)
%  % use tabular for content to get columns/rows
%  % parbox to limit width of the listing
%  \node[state, anchor=center] (S1) 
%  {Line 1, $[0,0]$};
%   
%  \node[state] (S2) [below =of S1]
%  {Line 2, $[0,0]$};
%  
%  \node[state] (S3) [below=of S2]
%   {Line 3, $[0,0]$};
% 
%  \node[state] (S4) [below =of S3]
%   {Line 1, $[1,1]$};
% 
%  \node[state] (S5) [below =of S4]
%   {Line 2, $[1,1]$};
% 
%  \node[state] (S6) [below =of S5]
%   {Line 3, $[1,1]$};
% 
% \node[state] (S7) [below =of S6]
%   {Line 1, $[2,2]$};
% 
% \node[state] (S8) [below =of S7]
%   {Line 1, $[1,\infty]$};
% 
% \node[nothing] (SN) [right =of S1]
%   {\Large{\dots}};
% 
% \node[state] (S8A) [below =of SN]
%   {Line 1, $[1,\infty]$};
% 
% \node[state] (S9) [below =of S8A]
%   {Line 2, $[1,\infty]$};
% 
% \node[state] (S10) [below =of S9]
%   {Line 3, $[1,\infty]$};
% 
% \node[state] (S11) [below =of S10]
%   {Line 1, $[2,\infty]$};
% 
% \node[state] (S12) [below =of S11]
%   {Line 1, $[1,\infty]$};
% 
% \node[nothing] (SN) [right =of S1]
%   {\Large{\dots}};
% 
%  % draw the paths and and print some Text below/above the graph
%  \path (S1) edge[right] node [below right] {} (S2)
%        (S2) edge[right] node [below right] {} (S3)
%        (S3) edge[right] node [below right] {} (S4)
%        (S4) edge[right] node [below right] {} (S5)
%        (S5) edge[right] node [below right] {} (S6)
%        (S6) edge[right] node [below right] {} (S7)
%        (S7) edge[right,dotted] node [dotted, below right] 
%             {$[1,1] \nabla ([1,1]\sqcup[2,2]) = [1, \infty)$} (S8)
% 
%        (S4) edge[ bend right=50,o->, dotted] node [right] {} (S8)
%        (S8A) edge[ bend left =50,o->, dotted] node [left] {} (S12)
% 
% 
%        (SN) edge[right] node [below right] {} (S8A)
%        (S8A) edge[right] node [below right] {} (S9)
%        (S9) edge[right] node [below right] {} (S10) 
%        (S10) edge[right] node [below right] {} (S11)
%        (S11) edge[right,dotted] node [below right,dotted] 
%             {$[1,\infty) \nabla ([1,\infty)\sqcup[2,\infty)) = [1, \infty)$} (S12);
% \end{tikzpicture}
% }
% \caption{Applying widening.}
% \label{fig:ex1_widen}
% \end{minipage}


The result of the construction is shown in Fig. \ref{fig:ex1_abstr}. The result is in general a 
\emph{Markov Decision Process}. 
Given a \emph{strategy} to resolve the nondeterminism, we obtain a Markov chain, 
for which we can compute the probability of reaching the fail location. The first theorem of our paper
is the counterpart of the result of \cite{kattenbelt,wachter} (when both are specialized to the 
particular case of sequential deterministic systems): the probability of reaching the fail
location in the Markov chain for the real program lies between the probabilities of reaching it under the
optimal and pessimal strategies for the MDP. Since these probabilities
can be computed using well-known algorithms, we obtain a lower and an upper bound for the real probability.
In our example we obtain a probability of failure of $0.01$, independently
of the strategy at the only nondeterministic state $\tup{1, [1, \infty]}$, and so we compute
the exact value. 

Actually, both our result and the result of \cite{kattenbelt,wachter} are stated for nondeterministic,
concurrent systems: in this general case, the semantics of the program is an MDP, the abstraction is
a 2-player stochastic game, and the result states that the probability of reaching a goal state in the 
program using an optimal strategy to resolve nondeterminism can be bounded from above and from below 
by computing the supremum and infimum of the probabilities of reaching the goal in the 2-player game 
when player 1 plays according to an optimal strategy (and player 2 is free to play in any way).

Consider now the program on the left of  Fig.~3, %%%!!!!!!!!!! MINIPAGE-REFERENZ! 
a variant of the program above. Here $\texttt{choice}(p)$ models a random number generator call, 
that returns $1$ with 
probability $p$ and $0$ with probability $1-p$. 

\begin{figure}[h]
\centering
\begin{minipage}[t]{0.45\linewidth} 
\label{fig:prog2}
 \begin{verbatim}
     int c = 0, i = 0;
  1: if choice(0.5) then
  2:   while (i <= 100) 
  3:     i = i+1;
  4:     c = c-i+2 
  5: if (c >= i) fail
 \end{verbatim}
\end{minipage}
\begin{minipage}[t]{0.45\linewidth} 
 \begin{verbatim}     
     int c = 0, i = 0;
  1: while(i <= 100) 
  2:   if choice(0.99) then i = (i+1);
  3:   c = c-i+2;
  4: if (c >= i) then fail
\end{verbatim}
\end{minipage}

\caption{Example programs 2 and 3.}
\end{figure}

It is easy to see that $c \leq 1$ is a global invariant, and so the probability of failure is exactly $0.5$. 
However, when this program is analyzed with PASS \cite{wachter,hermanns}, a leading tool on probabilistic 
abstraction refinement on the basis of predicate abstraction, the while loop is (implicitly) 
\andreas{implicitly eingefuegt, PASS kennt keine Schleifen} 
unrolled 100 times because the tool fails to ``catch'' the invariant, independently of the options chosen to 
refine the abstraction. On the other hand, an analysis of
the program with the standard interval domain, the standard widening operator, and the standard technique of delaying
widenings \cite{astree}, easily `catches'' the invariant (see Section \ref{sec:experiments} for a detailed analysis).
The same happens for the program on the right of the figure, which exhibits a more interesting probabilistic
behaviour: we obtain good upper and lower bounds for the probability of failure using the standard interval domain.

Notice that examples exhibiting the opposite behaviour (predicate abstraction succeeds where 
interval analysis fails) are not difficult to find. Our thesis is only that the MDP-based abstraction 
approach of \cite{kattenbelt,wachter} can be easily extended to arbitrary abstract domains, making it more flexible
and efficient.




